Efficient Bayesian estimation and use of cut posterior in semiparametric hidden Markov models

We consider the problem of estimation in Hidden Markov models with finite state space and nonparametric emission distributions. Efficient estimators for the transition matrix are exhibited, and a semiparametric Bernstein-von Mises result is deduced. Following from this, we propose a modular approach using the cut posterior to jointly estimate the transition matrix and the emission densities. We derive a general theorem on contraction rates for this approach. We then show how this result may be applied to obtain a contraction rate result for the emission densities in our setting; a key intermediate step is an inversion inequality relating $L^1$ distance between the marginal densities to $L^1$ distance between the emissions. Finally, a contraction result for the smoothing probabilities is shown, which avoids the common approach of sample splitting. Simulations are provided which demonstrate both the theory and the ease of its implementation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
